Model Checking Implantable Cardioverter Defibrillators

Ventricular Fibrillation is a disorganized electrical excitation of the heart that results in inadequate blood flow to the body. It usually ends in death within seconds. The most common way to treat the symptoms of fibrillation is to implant a medical device, known as an Implantable Cardioverter Defibrillator (ICD), in the patient's body. Model-based verification can supply rigorous proofs of safety and efficacy. In this paper, we build a hybrid system model of the human heart+ICD closed loop, and show it to be a STORMED system, a class of o-minimal hybrid systems that admit finite bisimulations. In general, it may not be possible to compute the bisimulation. We show that approximate reachability can yield a finite simulation for STORMED systems, which improves on the existing verification procedure. In the process, we show that certain compositions respect the STORMED property. Thus it is possible to model check important formal properties of ICDs in a closed loop with the heart, such as delayed therapy, missed therapy, or inappropriately administered therapy. The results of this paper are theoretical and motivate the creation of concrete model checking procedures for STORMED systems.

==> collectionSeparability.tex <==
\yhl{{\large \textbf{An equivalent characterization of Collection Separability}.}
	\\
Collection separability (Thm. \ref{thm:SHS composition}) can be equivalently expressed in terms of set operations. 
Let $R$ be the reachable set of $\Sys$,
and let $R_{|ij}$ be the projection of $R$ onto the space $\stSet^i \times \stSet^j$.
Then Collection Separability is expressed as:
\\
for all $i,j \leq m, i\neq j$ there exists $d_{min}^{ij}>0$ s.t. for all guards $\guard^i$ of $\Sys_i$ and all guards $\guard^j$ of $\Sys_j$, \begin{equation*}
R_{|ij} \cap \guard^i \times (\stSet^j \setminus \guard^j) \subset \stSet^i \times \{x^2 \in \stSet^2 \;|\; d(x^2,\guard^2) > d_{min}^{ij}\}
\end{equation*}}

==> formalOminimal.tex <==
\textbf{Formal definitions}.
A \emph{language} is a set of relations, functions and constants.
E.g. $\Lc_\Re = (<,+,-, \cdot,\Re)$ is the language where the only relation is $<$, the functions are $+,-,\cdot$, and the constants are taken from $\Re$,
and  $\Lc_{exp} = (<,+,-, \cdot,\exp, \Re)$ adds the exponential symbol to it.
Let $\Vc = \{x,y,z,x_1,x_2,\ldots\}$ be a set of variables.
A \emph{term} of a language is either a variable, a constant, or $F(\theta_1,\ldots,\theta_m)$ where $F$ is an $m$-ary function expressible in the language and the $\theta_i$ are terms.
E.g. $2x-3.6y$ is a term of $\Lc_\Re$.
The \emph{atomic formulas} of the language are of the form $\theta_1=\theta_2$ or $R(\theta_1,\ldots,\theta_m)$ where $R$ is an $m$-ary relation on the terms $\theta_i$.
E.g., $2x-3.6y < z\cdot z$ is a an atomic formula in $\Lc_\Re$ which uses the terms $2x-3.5y$ and $z \cdot z$.
The set of (first-order) \emph{formulas} is defined recursively as follows: every atomic formula is a formula, and if $\formula_1,\formula_2$ are formulas, then so are $\formula_1 \land \formula_2, \neg \formula_1, \forall x: \formula_1, \exists x:\formula_1$.
Here the symbols are the usual boolean connectives ( conjunction $\land$ and negation $\neg$), and quantifiers (there exists $\exists$ and for all $\forall$).
A \emph{sentence} in the language is a formula where all variables are inside the scope of a quantifier, e.g. $\exists y . (x+y>3)$ is not a sentence.

So far, a language has been defined in a purely syntactic manner.
A \emph{model} of a language is a set $S$ along with an interpretation of the relations, functions and constants of the language.
We are interested in this paper in the model of $\Lc_{exp}$ where the set $S = \Re$, and the symbols $<,+,-, \cdot,exp$ have their usual meaning (less than, addition, etc).
A set $Y \subset \Re^n$ is \emph{definable} in $\Lc_\Re$ if there exists a formula of the model such that $Y$ can be expressed as $Y = \{(a_1,\ldots,a_n) \in \Re^n \;|\; \formula(x_1,\ldots,a_n)\}$.
E.g., the formula $x^2-1=0$ defines the set $\{-1,+1\}$.
Finally, a \emph{theory} is a subset of sentences in the model $\Lc_\Re$, i.e. it is a collection of sentences that are true in $\Lc_\Re$.

==> properties.tex <==
\section{Properties of interest}
\label{sec:properties}
The finite simulation we obtain by running (the approximate version of) Alg.~\ref{algo:bisimulation} abstracts away the duration of continuous transitions $\trans{\tau}$, so that only time-unbounded properties (like LTL) can be verified on the abstraction.
%A priori, this is a shortcoming of the approach because many properties of interest for ICDs involve bounds on when events happen. 
However, every component of $\Sys_{ICD}$ has a local clock in its state vector.
Thus these clocks can be used to express interesting time-bounded properties of $\Sys_{ICD}||\Sys_{CA}$.

For example, to expresses that a Sustained \ac{VT} event should be followed by a \ac{VT} determination within 30sec, we write:
\begin{equation}
\label{eq:fTh}
\formula_{Th} \defeq \formula_{VT} \implies \formula_{VT} \until_{[0,30]} \Sys_{ICD}.Mode = VT
\end{equation}
The VT decision ($\Sys_{ICD}.Mode = VT$) can be reached by one of three paths of execution (see Fig. \ref{fig:bsc detection}):
For example, path $P_1$ goes from the root to ``8/10 faster'' on the right and ends in VT.
Along each path, the component automata have local clocks that keep track of how long they are running in this execution.
Therefore, the total execution time of all automata on a given path must be less than 30sec.
So the time constraint may now be expressed as the disjunction $\lor_{P \in \{P_1,P_2,P_3\}}\sum_{c\in P} c \leq 30$.
The formula can be re-written
\begin{equation*}
\formula_{VT} \implies \formula_{VT}\until \lor_{k=1,2,3}(\Sys_{ICD}.Mode = VT_k \land \sum_{c \in P_k} c \leq 30)
\end{equation*}
where $VT_k$ is the VT decision reached along the $k^{th}$ path.
%

%Letting VD denote a spontaneous (non-conducted) Ventricular Depolarization, the following formula describes a sequence of ventricular depolarizations that are 200ms or less apart.
%\begin{equation}
%\formula_{VF} \defeq VD \land \eventually_{[0,200]} (VD \land \eventually_{[0,200]} (VD \ldots))
%\end{equation}

%In terms of our model, a ventricular depolarization can be described as follows.
%Let $\Cc$ be a set of ventricular cells in the heart model that are meant to be the source of the depolarization, and let $\Nc(\Cc)$ be a neighborhood of these cells.
%The following expresses that the neighborhood is quiescent until the cells in $\Cc$ become active, implying spontaneous activity.
%Incidentally, this is a formula that does \emph{not} require time bounds, and so can be directly expressed in LTL.
%\begin{equation}
%VD \defeq \land_{c \in \Nc} (c.Mode = Quiescent) \until \land_{c\in \Cc} (c.Mode = Upstroke)
%\end{equation}
%Other ways of describing this event may be possible or preferable based on other factors.
%
%\todo[inline]{cite GF, Donze?}
%Signals used in TFL properties are also o-minimal (if the underlying time-domain signal is o-minimal), thus TFL properties can also be verified.
%Indeed, TFL properties use the Short-Time Fourier Transform (STFT) coefficients of the signal $x(t)$ to define predicates ($i=\sqrt{-1}$):
%\begin{eqnarray*}
%c_\omega(\tau) &=& \int_{\tau-L/2}^{\tau+L/2}x(t)g_L(t-\tau)e^{-i2\pi\omega t}dt
%\\
%&=& \int_{\tau-L/2}^{\tau+L/2}x(t)g_L(t-\tau)cos{2\pi\omega t}dt 
%\\
%&\quad& - i\int_{\tau-L/2}^{\tau+L/2}x(t)g_L(t-\tau)sin{2\pi\omega t}dt 
% \\
% &=& C_r(\tau+L/2) - C_r(\tau-L/2) 
% \\
% &\;& - i[C_i(\tau+L/2) - C_i(\tau - L/2)]
%\end{eqnarray*}
%Each of the summands is an integral. 
%The integrand in each is the product of a definable $x(t)$ and an analytic bounded $cos$ or $sin$ (bounded because multiplied by the window function $g_L$ of width $L$), and therefore it is definable. 
%So the antiderivatives $C_r,C_i$ are definable by a corollary of Spessegger \cite{Speissegger99_Pfaffian}.
%%($I \supset [\tau-L/2,\tau+L/2], a=\tau-L/2$), 
%So the real and imaginary parts of $c_\omega(\tau)$ are definable.
%If we identify the complex field $\Ce$ with $\Re^2$ and map the field operations of $\Ce$ to those of $\Re^2$ in the usual way, then $\Ce$ and its field operations are definable in $\Re$ and every algebraic subset of $\Ce^n$ is definable in $\Re$ \cite{PeterzilS04_ComplexOminmal}.
%Thus the function $\tau \mapsto c_\omega(\tau)$ is o-minimal being the result of applying multiplication (by $i$) and addition to definable terms.

==> simulationAprox.tex <==
\section{Finite simulation for STORMED systems}
\label{sec:simulationAprox}
%In general it is not possible to compute the bisimulation exactly unless the underlying o-minimal theory is decidable
Whether the bisimulations of STORMED systems can be computed depends on whether the underlying o-minimal theory is decidable. 
The human heart+ICD closed loop is definable in $\Lc_{exp}$, and the latter is not known to be decidable.
The authors in \cite{PrabhakarVVD09_toklerant} proposed approximating the flows and resets by polynomial flows and resets.
However, the process of approximation is typically iterative and requires manual intervention, or is restricted to subclasses of STORMED systems \cite{PrabhakarVVD09_toklerant}.
%More generally, building the abstraction might require explicit knowledge of the flows (solutions of the ODEs), which is often not possible.
%Collocation methods are more automatic and work with the ODEs directly, but they are restricted to sub-classes of STORMED systems and might still require manual intervention \cite{PrabhakarVVD09_toklerant}.
Even if the o-minimal theory is decidable, the decision procedure first applies Quantifier Elimination, whose worst-case time complexity is doubly exponential in the number of quantifier blocks \cite{DavenportH88_QE}.
%
Here we show that if an approximate reachability tool is available, it can be used in Algo~\ref{algo:bisimulation} (instead of exact reachability) to yield a \emph{finite simulation} (rather than a bisimulation).
%This is in the spirit of tolerant systems \cite{PrabhakarVVD09_toklerant}, but does not need explicit approximation of the flows.
%We take as our starting point the operators $\Fd$ and $\Fc$, and simply replace the exact $\Ft$ operator by an approximate operator $\Ft^\epsilon$ based on approximate reachability $\Rc^\epsilon_I$, as shown in the following Algorithm \ref{algo:apx Ft}.
%\begin{algorithm}
%	\caption{Simulation refinement for continuous transitions}
%	\label{algo:apx Ft}
%	\begin{algorithmic}
%		\Require Hybrid system $\Sys$, interval $I \subset [0,+\infty)$, a partition $\partition$ of $\hsSet$, $\epsilon>0$.
%		\State Set $\simu = \partition$			
%		\While{$\exists P,P' \in \simu$ s.t. $\emptyset \neq P' \cap \Rc^\epsilon_I(P) \cap P' \neq P'$}
%			\State Set $\simu = \simu \setminus \{P'\} \cup \{P' \cap \Rc_I^\epsilon(P) , P' \setminus \Rc_I^\epsilon(P) \}$
%		\EndWhile	
%		\State Return $\simu^\epsilon$
%	\end{algorithmic}
%\end{algorithm}
%It is clear that $\simu^\epsilon$ is a partition that refines $\partition$. 
%\begin{lemma}
%$\simu^\epsilon$ is finite.
%\end{lemma}
\begin{lemma}
	\label{lemma:finite simu}
	Let $\SHS = (\Sys,\ldots)$ be a SHS and $\partition$ a partition of $\stSet$.
	For any mode $\mode$ of $\Sys$ with flow $\theta_\mode $, consider the dynamical system $\Dc$ with state space $X = \Sys.\stSet$ and whose flow $\Theta: \Re \times \Re^n \rightarrow 2^{\Re^n}$ is a set-valued $\varepsilon$ over-approximation of $\theta_\mode$:
	$\Theta(t;x) = \{y \in \Re^n \;|\; ||y-\theta(t;x)||^2 \leq \epsilon^2\}$.	
	Then $\Dc$ admits a finite simulation $\simu_\mode$ that refines $\partition$, returned by Alg.~\ref{algo:bisimulation}.
\end{lemma}
The proof is in the Appendix.
%====================================================================================
%This finite simulation is that returned by running Algorithm 1 with the approximate reachability. 
%The lemma can be repeated for all modes of $\Sys$ producing a simulation $\simu_\mode$ for each mode $\mode \in \modeSet$.
Let $\Ft^\epsilon(\partition) \defeq \cap_{\mode}\simu_{\mode \in \modeSet}$: then it refines all the $\simu_\mode$'s, and it is a finite simulation of $\Sys$ by itselt w.r.t. the continuous transition $\trans{\tau}$.
%Let $\simue$ be the finite simulation of $\Sys$ thus obtained, and let $\partition_{\simue}$ be the associated partition of $\hsSet$.
%$\Ft^\epsilon(\partition) \defeq \{(\stPt,P)  \in \hsSet \times \simu^\epsilon \;|\; \stPt \in P\}$.
It is clear that $\Ft^\epsilon(\cdot)$ is idempotent: $\Ft^\epsilon(\Ft^\epsilon(\partition)) = \Ft^\epsilon(\partition)$
%We also have:
%\begin{lemma}
%For any partition $\partition$, $\Ft^\epsilon(\partition)$ is a simulation of $\Sys$ by $T_\Sys/\simu^\epsilon$.
%\end{lemma}
%\begin{proof}
%Two states $x,x' \in \stSet$ are related by $\simu^\varepsilon$ iff $q(x) = q(x')$, that is, their flows visit the same sequence of blocks of $\partition$.
%Do they also visit the same sequence of blocks in $\partition_{\simue}$?
%Assume not, and let $B,B' \in \partition_{\simue}$ be the first blocks in which they differ, that it, $\theta(x,t) \in B$ and $\theta(x',t) \in B'$.
%Because $B,B'$ are different blocks, this implies that there exist $y\in B,y' \in B'$ such that $q(y) \neq q(y')$.
%But $x \in B \implies q(x) = q(y)$, and similarly $x' \in B' \implies q(x')=q(y')$, which contradicts $q(x) = q(x')$.
%Therefore the flows of $x$ and $x'$ visit the same sequence of blocks in $\partition_{\simue}$.
%Thus if we re-apply $\Ft^\varepsilon$ to $\simu^\varepsilon$, it will again yield $x$ and $x'$ will again have the same strings and so remain related by $\Ft^\varepsilon()$
%%Idempotency is immediate: Algorithm \ref{algo:apx Ft} terminates only when no further partitioning of any block $P$ is possible. Thus if we re-run it on $\simu^\epsilon$, it will return $\simu^\epsilon$ and the resulting relation $\Ft^\epsilon$ is unchanged.
%
%Let $\simu^\epsilon = \{P_1,\ldots,P_V\}$ be the final refinement of $\partition$ returned by Algorithm \ref{algo:apx Ft}.
%Write $F \defeq \Ft^\epsilon(\partition)$.
%Let $(x,P) \in F$, that is, $x \in P$. 
%Consider a continuous transition $x \trans{\tau} y$ such that $y = \theta(x,t)$.
%Then by definition $y \in \Theta(x,t) \subset P'$ for some $P' \in \simu^\epsilon$. 
%Moreover $P \trans{} P'$ by definition of the transition relation of $T_\Sys/\simu^\epsilon$, so $(y', P') \in F$.
%
%The converse is not necessarily true: if $P \trans{}P'$ then it might be that $P' = \Rc^\epsilon_I(P) \setminus \Rc^0_I(P)$, i.e. $P'$ is purely the result of the over-approximation.
%In this case, it can not be guaranteed that $x \in P$ will evolve into $P'$.
%This is why $\Ft^\epsilon$ is only a simulation.
%\end{proof}

%====================================================================================

\begin{thm}
	\label{thm:finite simulation}
	Let $\Sys$ be a STORMED hybrid system, 
	and $\partition$ be a finite definable partition of its state space.
	Define 
	\begin{compactitem}
		\item $W_0 = \Ft^\epsilon(\partition)$.
		\item For all $i\geq 0$, $W_{i+1} = \Ft^\epsilon(\Fd(W_i))$.
	\end{compactitem}
Then there exists $U \in \Ne$ s.t. $W_{U+1} = W_U$ and $\Ft^\epsilon(W_U)$ is a simulation of $\Sys$ by itself.
\end{thm}

\begin{prf}
By Lemma 10 of \cite{VladimerouPVD08_STORMED} there exists a uniform bound $U$ on the number of discrete transitions of any execution of the STORMED system $\Sys$, so $\Fd(W_k) = W_k$ for all $k\geq U$.
Moreover 
$W_{U+1} = \Ft^\epsilon(\Fc_d(W_U)) = \Ft^\epsilon(W_U)$
and $W_{U+2}= \Ft^\epsilon(\Fc_d(W_{U+1}))= \Ft^\epsilon(\Fc_t(W_U)) = \Ft^\epsilon(W_U) = W_{U+1}$, so the iterations reach a fixed point.
The fact that $\Ft^\epsilon(W_U)$ is a simulation then yields the desired result.
\end{prf}
%
%Let $AP$ be a set of atomic propositions, and let $\formula$ be an LTL formula over $AP$.
%If the initial partition $\partition$ we start with is given by $x \equiv_\partition y$ iff $(x \models p \leftrightarrow y \models p \; \forall p \in AP)$, then the fact that simulation $\Sys^\epsilon$ satisfies $\formula$ implies that the original hybrid system $\Sys$ satisfies it too. 
\input{spaceex}



==> spaceexDef.tex <==
{\large \textbf{Proof of Thm.~\ref{thm:spaceex definable}}.}
\begin{prf}
	\newcommand{\EPS}{\mathcal{E}}
	We show that if $S \subset \Re^n$ is o-minimal, then $\boxdot S$ and $TH_\Vc(S)$ are o-minimal. 
	O-minimality of the other sets is a standard result.
	
	We start with $\boxdot S$.
	\begin{eqnarray*}
		\boxdot S &=& \{y \in \Re^n \;|\; -\overline{|x_i|}\leq y_i \leq \overline{|x_i|},i=1,\ldots,n\}
		\\
		&=& \{y \in \Re^n \;|\; \exists a_i \in \Re_+. (a_i = \sup \{|x_i|,x\in S\} 
		\\
		&& \land (-a_i\leq y_i \leq a_i)),i=1,\ldots,n\}
		\\
		&=&  \{y \in \Re^n \;|\; \exists a_i \in \Re_+. (\forall \varepsilon_i>0 \exists x_i \in S . a_i-\varepsilon < |x_i(i)|)
		\\
		&& \land (-a_i\leq y_i \leq a_i)),i=1,\ldots,n\}
		\\
		&=&  \{y \in \Re^n \;|\; \exists a_i \in \Re_+. (\forall \varepsilon_i>0 \exists x_i \in S . a_i-\varepsilon < x_i(i)
		\\
		&& \lor a_i - \varepsilon > -x_i(i)) \land (-a_i\leq y_i \leq a_i)),i=1,\ldots,n\}
\end{eqnarray*}

The template hull is given by
\[TH_\Vc(X) \defeq \{x\in\Re^n \;|\;\land_{a \in \Vc} a\cdot x \leq \rho(a,X)\}\]
where the support function is given by 
\begin{equation}
\label{eq:supportfnt}
\rho(a,S) \defeq \max_{x \in S} a\cdot x
\end{equation}
Therefore $TH_\Vc(X)$ is definable if $\rho$ is.
The graph of $a \mapsto \rho(a,S)$ is given by 
\begin{eqnarray}
\textbf{Gph}\rho = \{(a,r) \;|\; \forall x\in S.\; r\geq a\cdot x \land \exists x\in S. r=a\cdot s\}
\end{eqnarray}
which is a first-order formula on predicates that use $+,\times$.
Since $S$ is o-minimal, Gph$\rho$ is o-minimal.
%
%To do so we show that it can be computed using a finite number of operations from the o-minimal structure $\Lc_{\exp}$.
%As we assume that $S$ is a polytope (a closed bounded intersection of half-spaces), it has a finite number of extreme points. 
%Let $\mathcal{E} =  \{e_i,i=1,\ldots,k\}$ be the set of extreme points and any point $x\in S$ can be written as a convex combination of the extreme points: $x = \sum_{i}\alpha_i e_i$.
%Therefore we can write
%\[ \rho(a,S) = \max_{\alpha \in I^k} \sum_{i=1}^k \alpha_i a\cdot e_i \]
%where $I^k = \{(\alpha_1,\ldots,\alpha_k)\;|\; \alpha_i \geq 0, \sum \alpha_i = 1\}$
%
%The maximizer $x^*$ of \eqref{eq:supportfnt} is necessarily a boundary point of $S$.
%Indeed let $x^0$ be an interior point of $S$ ($x^0 \in S\setminus \partial S$).
%Then the line through $x^0$ intersects $\partial S$ twice, at points $\lambda_1x^0$ and $\lambda_2x^0$, with $\lambda_1 \geq 1$ and $\lambda_2 \leq 1$.
%This is the case because $S$ is closed and bounded.
%If $a\cdot x^0 \geq 0$, then $a\cdot \lambda_1 x^0 \geq a\cdot x^0$. 
%And if $a\cdot x^0<0$ then $0 \geq a\cdot \lambda_2 x^0 \geq a\cdot x^0$. 
%Thus to any interior point of $S$ there exists a boundary point with a larger projection on $a$.
%
%A boundary point can always be written as the convex combination of exactly $n$ extreme points, namely the extreme points that are the vertices of the face to which the boundary point belongs.
%
%Therefore the support function expression is further simplified to:
%\[ \rho(a,S) = \max_{\alpha \in [0,1], \mathcal{F} \subset \EPS:|\mathcal{F}|=n } \sum_{i=1}^n \alpha_i a\cdot e_i \]
	\end{prf}

==> statementOfResults.tex <==
\section{Statement of results}
\label{sec:stmt}
state main results here in compact form
